NVIDIA Spectrum-X: Hardware-Accelerated Multiplane Networking for Large-Scale AI Training

As distributed model training scales to span hundreds of thousands of GPUs, scale-out networks face unprecedented performance and efficiency demands. NVIDIA Spectrum-X Ethernet has been designed from the ground up to achieve predictable and stable network performance with high utilization and low latency. This paper presents the Spectrum-X multiplane architecture, which replaces hierarchical depth with topological parallelism, and introduces hardware-accelerated load balancing in NICs and switches as the key architectural approach to provide fast reaction to highly dynamic network conditions at the microsecond timescales that AI training workloads demand. We describe the motivation, design principles, evaluation methodology and performance on state-of-the-art benchmarks, as well as the lessons we learned from deploying and debugging Spectrum-X networks in large-scale systems. Our evaluation highlights production-grade AI infrastructure performance across four core dimensions: 98% of the theoretical line rate with low jitter-free latency; strong cross-tenant isolation for concurrent workloads; robust, capacity-proportional bisection bandwidth and 7% latency increase for 10% fabric link failures; and rapid reaction to host and fabric link flaps during LLM training workloads.

==> Reviews_and_requests.tex <==
R1: 

The paper claims PFC storms don’t occur. Can you address tenant isolation? In my experience, a badly written application can cause GPU memory system to back up and PFCs from NICs. In a multi-tenant environment that could cause performance degradation to other tenants.
\textbf{>> Address tenant isolation with clients who cause PFC storms}
* Answer: ??

Section 4.2 claims ECN marks only when LB capacity is exhausted, Cannot it happen during incast?

*Fixed*

Section 4.4, Resilience. How about reaction to remote link failures? Table 1 states millisecond reaction. Is it good-enough? 
* Answer:  we see that this is not a problem in our experiments.

Section 5.1 states that symmetry is expected in per-link BW. why? How about irregular topologies due to faults? Related work: Falcon’s multipathing separates CC per-path.
* Answer:  we do not address that


Editorial comments

Figures 1-3 appear in page 4 while being referenced in page 2 and 3.
* Fixed

Section 2.1, describing jitter as inter-collective and intra-collective interference is a little strange. Better describe it as self-inflicted (all-to-all) and interference based queuing (lack of perfect load-balancing)
* Disagree, not addressed

Section 3.2 mentions congestion control is only triggered by incast without saying how given the signal is delay. 
* unclear comment

Section 3.2 Ethernet/TCP/IP/BGP seems like a soup of protocols rather than a particular solution.
*Fixed

Figure 3 text is too small.
* Fixed

Sec 5.2, SPX hardware exposes per-usec histogram. Which HW? NIC or Switch or both. Please clarify.
*Fixed

Sec 5.3 says middle graph. I see only two graphs a and b. Please fix.
*Fixed

====


\subsubsection{Recommended Revisions}


C1, C2, C3 are unaddressable IMHO.

\begin{enumerate}
    \item Clarify the paper's positioning against recent production multiplane AI fabrics, such as Alibaba HPN and Tencent Astral, using explicit comparison criteria rather than only naming related systems.
    \item Provide more concrete detail on the congestion-control and PLB mechanisms, including key algorithms/parameters, convergence behavior, PLB state lifetime/reset behavior.
\end{enumerate}


\subsubsection{Comments for authors}


C1. This comment expands on the first recommended revision above. The paper should more clearly position SPX against recent production AI fabrics such as Alibaba HPN and Tencent Astral, as well as the closely related MIT/Meta Rail-only design. HPN and Astral use multi-plane-like designs, and Rail-only explores an adjacent rail-based design point, even if these works do not define "multiplane" exactly as SPX does. A useful comparison would use explicit criteria such as topology, load-balancing and congestion-control schemes, failure handling, diagnosability, and operational complexity, rather than only naming related systems. The goal is not necessarily to require full head-to-head experiments, but to help readers understand the novelty and production experience.

C2. The paper should also clarify how its congestion-control and load-balancing algorithms relate to prior mechanisms such as MRC, UET, SGLB, DCQCN, and Swift. This comparison would help readers understand the similarities and differences between SPX and prior mechanisms, and clarify what evidence supports the claimed benefits of SPX's hardware control-loop decomposition. If certain head-to-head comparisons or ablations are infeasible, it would be helpful to state those limitations explicitly.

C3. The congestion-control and PLB mechanisms need more concrete algorithmic detail. Sections 4.2 and 4.3 describe the high-level design, but leave key parameters, rate update rules, PLB state lifetime/reset behavior, and convergence behavior unclear.

C4. There are some typos and wording issues:

\begin{itemize}

*** ADDRESSED ***

    \item Figure 3: "absurption" should be "absorption".
    \item Section 3: "Spectrum switches and ConnectX NIC's based AI solution architecture" should be rewritten, for example as "AI solution architecture based on Spectrum switches and ConnectX NICs".
    \item Section 3.1: "three-tier fat-trees" should be "three-tier fat-tree" or otherwise rephrased for agreement.
    \item Section 5.3: "HW accelearted HFT" should be "HW accelerated HFT".
    \item Section 6.1: "don't" should be replaced with "do not" in formal paper prose.
====
\item

** What are the specifics of the CC and the difference b/w per-plane and per flow CC. 

** How per-flow CC and per-plane CC interact. 

** How per-plane CNP is generation is realized? 

** how is the current transmission rate is determined when updating the CC per plane




However, the current version lacks several key details needed to fully understand and evaluate the design. My main concern is how per-plane congestion control and inter-plane load balancing effectively work together. Sections 4.2 and 4.3 provide an initial description of the design ideas, but many important design and implementation details are still missing.

For example, Section 4.2 only describes that the congestion control mechanism leverages ECN and RTT signals, but lacks details about the underlying algorithm. The paper claims that SPX supports both per-flow and per-plane congestion control. Are the CC algorithms used at these two granularities identical? There have been extensive studies on congestion control algorithms in the community; how does the CC design adopted by SPX compare with existing approaches in related work?

Furthermore, the paper should clarify the objectives and interactions between per-flow CC and per-plane CC.

How do these two mechanisms make decisions independently, and how are their decisions coordinated when they operate together? Since PLB also makes path-selection decisions, a clearer analysis of the coupling and trade-offs among congestion control and load balancing mechanisms would significantly strengthen the paper.

How per-plane CNP generation is realized? DCQCN uses a configurable interval to rate-limit CNP generation; it is unclear whether this interval is maintained globally, per QP, or per plane in SPX. If the mechanism is per-plane, how does the receiver identify the corresponding plane and maintain plane-specific congestion state?

Section 4.3 describes how SPX selects planes under CC rate limiting. It mentions comparing the CC rate allowance of each plane with the current transmission rate. However, it is unclear how SPX defines and estimates the current transmission rate. Since transmission rate is typically measured over a time window, additional details on how this metric is maintained and used would help clarify the design.

Misc: It is unclear how to interpret the experimental results in Figure 14(b). How should readers understand the results among different states (e.g., pristine, failed, and degraded)? In addition, what is the exact definition of convergence time in this experiment?
[ FIXED ]

\item ====

* How does SPX handle oversubscribed networks? 
* How does it handle oversubscribtion under failures?
* What is the precise CC algo? 4.2 need to be rewritten??
* If CC is per plane, is there per-QP CC as well? and CNP is generated per plane, won't it break fairness/isolation guarantees across QPs? They seem to be important properties to have, even in an AI cluster context.
* How does lesson learned section related to the design? 
* WHy were there not PFC storms? any evidence ? How do we know it will remain the same in the future. 

First, the design decision of having independent control loops for load balancing and end-point congestion control seems to be correct only for full-bisection bandwidth networks. Does that mean Spectrum-X is designed to work correctly only when there is no oversubscription? Also, even with full-bisection bandwidth networks, link failures in the leaf-to-spine layer could result in effective oversubscription, leading to in-network congestion even with perfect load balancing (and hence coupling end-to-end congestion control and load-balancing loops).

Second, it was hard to follow S4.2. Where exactly is SPX CC logic implemented? At each switch port NIC? If yes, I fail to understand the reasoning behind it and the mechanism as well (is it at a per-switch-hop level)? What is the precise CC algorithm? If this is a CC algorithm implemented at the end-host NICs, why is it discussed in the forwarding and load-balancing subsections (and is the discussion of NIC CC also present in the later subsections)? The text only mentions: “SPX CC combines RTT probes with explicit switch signals: ECN marks only when load-balancing capacity is exhausted, and CC reacts only to these signals as shown in Fig. 3. RTT then guides precise rate adjustment, maintaining high throughput and low latency.” At a high level, this just seems like DCQCN with a larger threshold. Anyways, this subsection requires clarification.

In S4.3, are NICs no longer performing per-QP congestion control and rate computation? From the description, it seems that CNP generation and rate computation are performed only on a per-plane basis. If this is true, won't it break fairness/isolation guarantees across QPs? They seem to be important properties to have, even in an AI cluster context.

Finally, the lessons learned from production experience seem quite thin (especially for an operational systems track paper, where I didn’t gain any particularly novel technical insights into the design). There is some discussion of High-Frequency Telemetry and its benefits for monitoring/debugging, with little introduction. I couldn’t understand exactly how it relates to the Spectrum-X design discussed earlier or to its deployment.

A nit: in S3.2 it is stated “PFC storms [18] are often cited as the argument against the use of lossless fabric. We observe no evidence of such storms in our own operational experience across more than two years of production operation of SPX deployed on the largest AI clusters.” It would be hard to buy this argument without providing more details on production experience. Maybe the workloads were not stressing the network enough? Moreover, the applications and workloads keep evolving. How do we know the statement will remain true in the near future?


==> figures/ballsinbins/production_data.tex <==
\begin{tikzpicture}
      \begin{axis}[
        width=\linewidth, height=5.5cm,
        ymode=log,
        x dir=reverse,
        xmin=69, xmax=101.5,
        xtick={70,75,80,85,90,95,100},
        xticklabels={70\%,75\%,80\%,85\%,90\%,95\%,100\%},
        xticklabel style={font=\footnotesize},
        ymin=0.8, ymax=200000,
        ytick={1,10,100,1000,10000,100000},
        yticklabels={1,10,100,1K,10K,100K},
        ylabel={Count leaf pairs},
        xlabel={Max-flow \% of full BW},
        xlabel style={font=\small},
        ylabel style={font=\small},
        title={\small\textbf{Leaf-to-Leaf Max-Flow Distribution}},
        grid=major,
        grid style={line width=0.3pt, draw=gray!40},
        legend style={
          font=\scriptsize,
          at={(0.97,0.97)},
          anchor=north east,
          fill=white, draw=gray!50,
          cells={anchor=west},
        },
      ]
        %% PHX61 2024-7-12  (bright green)
        \addplot[nvidia_green, line width=1.5pt, mark=*, mark size=1.5pt,
                 mark options={solid, fill=nvidia_green}] coordinates {
          (100,21898)(96.875,9168)(93.75,4791)(90.625,1550)
          (87.5,424)(84.375,147)(81.25,31)(78.125,11)(75,2)
        };
        \addlegendentry{PHX61 2024-7-12}
        \addplot[nvidia_green, draw=none, mark=none, forget plot,
                 nodes near coords, nodes near coords align={anchor=south},
                 every node near coord/.append style={font=\scriptsize, color=nvidia_green!80!black, inner sep=3pt, xshift=4pt},
                 point meta=explicit symbolic,
        ] coordinates { (100,21898) [21898] };
        \addplot[nvidia_green, draw=none, mark=none, forget plot,
                 nodes near coords, nodes near coords align={anchor=north},
                 every node near coord/.append style={font=\scriptsize, color=nvidia_green!80!black, inner sep=3pt, xshift=-4pt},
                 point meta=explicit symbolic,
        ] coordinates {
          (90.625,1550) [1550]
          (81.25,31)    [31]
        };
        \addplot[nvidia_green, draw=none, mark=none, forget plot,
                 nodes near coords, nodes near coords align={anchor=north},
                 every node near coord/.append style={font=\scriptsize, color=nvidia_green!80!black, inner sep=3pt, xshift=-4pt, yshift=2pt},
                 point meta=explicit symbolic,
        ] coordinates { (75,2) [2] };

        %% PHX11 2024-8-7  (dark green)
        \addplot[nvidia_green!50!black, line width=1.5pt, mark=square*, mark size=1.5pt,
                 mark options={solid, fill=nvidia_green!50!black}] coordinates {
          (100,6206)(96.875,6462)(93.75,4199)(90.625,2005)
          (87.5,1037)(84.375,390)(81.25,129)(78.125,16)(75,3)(71.875,1)
        };
        \addlegendentry{PHX11 2024-8-7}
        \addplot[nvidia_green!50!black, draw=none, mark=none, forget plot,
                 nodes near coords, nodes near coords align={anchor=north},
                 every node near coord/.append style={font=\scriptsize, color=nvidia_green!50!black, inner sep=3pt, xshift=4pt},
                 point meta=explicit symbolic,
        ] coordinates { (100,6206) [6206] };
        \addplot[nvidia_green!50!black, draw=none, mark=none, forget plot,
                 nodes near coords, nodes near coords align={anchor=south},
                 every node near coord/.append style={font=\scriptsize, color=nvidia_green!50!black, inner sep=3pt, xshift=4pt},
                 point meta=explicit symbolic,
        ] coordinates {
          (90.625,2005) [2005]
          (81.25,129)   [129]
          (75,3)        [3]
        };
      \end{axis}
    \end{tikzpicture}

==> figures/ballsinbins/simulation_histogram.tex <==
%%=================================================================
%% figures/ballsinbins/simulation_histogram.tex
%% Monte Carlo simulation: common uplinks per leaf pair
%% Topology: 256 leaves x 128 spines, 2000 experiments (seeds 42, 123)
%%=================================================================

\begin{tikzpicture}
  \begin{axis}[
    width=\linewidth, height=5.5cm,
    ymode=log,
    x dir=reverse,
    xmin=72.5, xmax=101,
    xtick={75,80,85,90,95,100},
    xticklabels={75\%,80\%,85\%,90\%,95\%,100\%},
    xticklabel style={font=\footnotesize, rotate=30, anchor=east},
    ymin=0.001, ymax=25000,
    ytick={0.01,0.1,1,10,100,1000,10000},
    yticklabels={0.01,0.1,1,10,100,1K,10K},
    ylabel={Average leaf pair count},
    xlabel={Max-Flow Percentage},
    xlabel style={font=\small},
    ylabel style={font=\small},
    title={\small\textbf{Leaf-to-Leaf Max-Flow Distribution}},
    grid=major,
    grid style={line width=0.3pt, draw=gray!40},
    legend style={
      font=\scriptsize,
      at={(0.97,0.97)},
      anchor=north east,
      fill=white, draw=gray!25, line width=0.3pt,
      cells={anchor=west},
      inner sep=1.5pt,
    },
  ]

    \addplot[light_green, line width=1.5pt,
             mark=*, mark size=1.5pt, mark repeat=3,
             mark options={solid, fill=light_green}]
      table[x=pct, y=fr_1, col sep=comma]
      {figures/ballsinbins/histogram_256l_128s_data.csv};
    \addlegendentry{1\% failure}

    \addplot[nvidia_green, line width=1.5pt,
             mark=square*, mark size=1.5pt, mark repeat=3,
             mark options={solid, fill=nvidia_green}]
      table[x=pct, y=fr_2, col sep=comma]
      {figures/ballsinbins/histogram_256l_128s_data.csv};
    \addlegendentry{2\% failure}

    \addplot[dark_green, line width=1.5pt,
             mark=triangle*, mark size=1.5pt, mark repeat=3,
             mark options={solid, fill=dark_green}]
      table[x=pct, y=fr_3, col sep=comma]
      {figures/ballsinbins/histogram_256l_128s_data.csv};
    \addlegendentry{3\% failure}

    \addplot[nvidia_green!60!black, line width=1.5pt,
             mark=diamond*, mark size=1.5pt, mark repeat=3,
             mark options={solid, fill=nvidia_green!60!black}]
      table[x=pct, y=fr_4, col sep=comma]
      {figures/ballsinbins/histogram_256l_128s_data.csv};
    \addlegendentry{4\% failure}

    \addplot[dark_gray, line width=1.5pt,
             mark=otimes*, mark size=1.5pt, mark repeat=3,
             mark options={solid, fill=dark_gray}]
      table[x=pct, y=fr_5, col sep=comma]
      {figures/ballsinbins/histogram_256l_128s_data.csv};
    \addlegendentry{5\% failure}

  \end{axis}
\end{tikzpicture}


==> figures/failures/allgather_failures.tex <==
\begin{tikzpicture}
  \begin{axis}[
      nccl axis, 
      xmode=log,
      width=\linewidth,
      height=0.4\linewidth, 
      ymax=60, 
      xmin=90000, 
      xmax=2e10,
      % Override the y-ticks from the base style to fit ymax=60
      ytick={0, 20, 40, 60},
      tick label style={font=\scriptsize},
      label style={font=\footnotesize},
      legend style={
        font=\scriptsize,
        at={(0.02,0.98)}, 
        anchor=north west,
        fill=white,
        fill opacity=0.9,
        draw=gray!50,
      },
  ]

  % 1. Pristine (Solid, Light Blue)
  % Plotted first so it sits underneath the dashed line
  \addplot[
    color=nvidia_green,
    solid, % Explicitly solid
    line width=1.5pt,
    mark=*,
    mark size=1.2pt,
    mark options={solid, fill=nvidia_green},
  ] coordinates {
    (130560,0.38) (262080,0.95) (524160,1.83) (1048320,4.35) (2096640,10.11) 
    (4194240,12.04) (8388480,18.7) (16776960,20.43) (33553920,30.48) 
    (67108800,42.04) (134217600,43.55) (268435200,46.83) (536870400,45.07) 
    (1073741760,46.79) (2147483520,47.32) (4294967040,47.49) (8.58993e9,47.4) 
    (1.71799e10,47.52)
  };
  \addlegendentry{Pristine}

  % 2. Failures (Dashed, Dark Blue)
  % Plotted second so the dashes sit on top
  \addplot[
    color=dark_gray,
    dashed, % Dashed line to show the overlap
    line width=1.5pt, 
    mark=square*,
    mark size=1.2pt, 
    % The marker outline is kept solid so the boxes don't get dashed borders
    mark options={solid, fill=white, draw=dark_gray, line width=1pt},
  ] coordinates {
    (130560,0.36) (262080,0.93) (524160,1.72) (1048320,4.24) (2096640,9.97) 
    (4194240,14.76) (8388480,18.67) (16776960,20.27) (33553920,30.34) 
    (67108800,42.04) (134217600,43.59) (268435200,46.83) (536870400,45.03) 
    (1073741760,46.74) (2147483520,47.33) (4294967040,47.5) (8.58993e9,47.4) 
    (1.71799e10,47.52)
  };
  \addlegendentry{Failures}

  \end{axis}
\end{tikzpicture}

==> figures/failures/allreduce_failures.tex <==
\begin{tikzpicture}
  \begin{axis}[
      nccl axis, 
      xmode=log,
      width=\linewidth,
      height=\linewidth, 
      ymax=400, % Bumped to 400 to fit the top tick
      xmin=90000, 
      xmax=2e10,
      ytick={0, 100, 200, 300, 400},
    xtick={131072, 67108864, 1.7179869184e10},
    xticklabels={128 KB, 64 MB, 16 GB},  
      tick label style={font=\scriptsize},
      label style={font=\footnotesize},
      legend style={
        font=\scriptsize,
        at={(0.02,0.98)}, 
        anchor=north west,
        fill=white,
        fill opacity=0.9,
        draw=gray!50,
      },
  ]

  % 1. Pristine (Solid, Light Blue)
  % Plotted first so it sits underneath the dashed line
  \addplot[
    color=nvidia_green,
    solid, % Explicitly solid
    line width=1.75pt,
    mark=*,
    mark size=1.5pt,
    mark options={solid, fill=nvidia_green},
  ] coordinates {
    (131072,1.44) (262144,2.23) (524288,5.54) (1048576,10.44) (2097152,19.11) 
    (4194304,33.0) (8388608,51.8) (16777216,75.31) (33554432,84.6) 
    (67108864,153.15) (134217728,209.13) (268435456,259.93) (536870912,295.28) 
    (1073741824,324.45) (2147483648,342.7) (4.29497e9,354.95) (8.58993e9,362.4) 
    (1.71799e10,366.86)
  };
  \addlegendentry{Pristine}

  % 2. Failures (Dashed, Dark Blue)
  % Plotted second so the dashes sit on top
  \addplot[
    color=dark_gray,
    dashed, % Dashed line to show the overlap
    line width=1.75pt,
    mark=square*,
    mark size=1.5pt,
    % The marker outline is kept solid so the boxes don't get dashed borders
    mark options={solid, fill=white, draw=dark_gray, line width=1.2pt},
  ] coordinates {
    (131072,1.43) (262144,2.44) (524288,5.49) (1048576,10.24) (2097152,20.25) 
    (4194304,33.04) (8388608,52.61) (16777216,73.83) (33554432,88.14) 
    (67108864,152.57) (134217728,208.86) (268435456,255.63) (536870912,294.2) 
    (1073741824,324.41) (2147483648,343.65) (4.29497e9,353.74) (8.58993e9,362.35) 
    (1.71799e10,366.82)
  };
  \addlegendentry{Failures}

  \end{axis}
\end{tikzpicture}

==> figures/failures/alltoall_failures.tex <==
\begin{tikzpicture}
  \begin{axis}[
      nccl axis, 
      xmode=log,
      width=\linewidth,
      height=\linewidth, 
      ymin=0, % Added this line to start y-axis at 0
      ymax=50, 
      xmin=90000, 
      xmax=2e10,
      ytick={0, 100, 200, 300, 400},
    xtick={131072, 67108864, 1.7179869184e10},
    xticklabels={128 KB, 64 MB, 16 GB},  
      ytick={0, 10, 20, 30, 40, 50},
      tick label style={font=\scriptsize},
      label style={font=\footnotesize},
      legend style={
        font=\scriptsize,
        at={(0.02,0.98)}, 
        anchor=north west,
        fill=white,
        fill opacity=0.9,
        draw=gray!50,
      },
  ]

  % 1. Pristine (Solid, Light Blue)
  % Plotted first so it sits underneath the dashed line
  \addplot[
    color=nvidia_green,
    solid, % Explicitly solid
    line width=1.5pt,
    mark=*,
    mark size=1.2pt,
    mark options={solid, fill=nvidia_green},
  ] coordinates {
    (130560,0.12) (261120,0.29) (522240,0.53) (1044480,1.29) (2096640,2.44) 
    (4193280,4.33) (8386560,7.96) (16773120,11.72) (33553920,17.2) 
    (67107840,30.19) (134215680,36.43) (268431360,39.74) (536870400,44.11) 
    (1073740800,45.61) (2147481600,45.11) (4294963200,45.17) (8.58993e9,46.19) 
    (1.71799e10,46.86)
  };
  \addlegendentry{Pristine}

  % 2. Failures (Dashed, Dark Blue)
  % Plotted second so the dashes sit on top
  \addplot[
    color=dark_gray,
    dashed, % Dashed line to show the overlap
    line width=1.5pt,
    mark=square*,
    mark size=1.2pt,
    % The marker outline is kept solid so the boxes don't get dashed borders
    mark options={solid, fill=white, draw=dark_gray, line width=1pt},
  ] coordinates {
    (130560,0.13) (261120,0.28) (522240,0.53) (1044480,1.13) (2096640,2.44) 
    (4193280,4.39) (8386560,8.67) (16773120,11.72) (33553920,16.93) 
    (67107840,30.09) (134215680,35.83) (268431360,39.69) (536870400,43.61) 
    (1073740800,45.37) (2147481600,44.88) (4294963200,45.22) (8.58993e9,46.27) 
    (1.71799e10,46.85)
  };
  \addlegendentry{Failures}

  \end{axis}
\end{tikzpicture}

==> figures/pgfplotset_definition.tex <==
\pgfplotsset{
  nccl axis/.style={
    width=0.4\textwidth,      % Scales the width
    height=0.28\textwidth,    % Keeps a good aspect ratio
    % Use scientific notation for xmin/xmax to avoid TeX overflow
    xmin=90000,
    xmax=2e10, 
    ymin=-7.897,
    ymax=191.577,
    xmode=log,
    % Remove top and right axis lines
    axis x line*=bottom,
    axis y line*=left,
    % Use scientific notation for ticks > 2.14 billion
    xtick={
      16384, 262144, 4194304, 67108864, 1073741824, 1.7179869184e10
    },
    xticklabels={
      16 KB, 256 KB, 4 MB, 64 MB, 1 GB, 16 GB
    },
    x tick label style={font=\footnotesize},
    ytick={0,25,50,75,100,125,150,175,200},
    y tick label style={font=\footnotesize},
    xlabel={Message size},
    ylabel={Bus bandwidth (GB/s)},
    label style={font=\fontsize{10}{10}\selectfont},
    grid=major,
    every major grid/.style={dashed, draw opacity=0.7},
    tick align=outside,
    legend style={
      font=\fontsize{9}{10}\selectfont,
      at={(0.99,0.02)},
      anchor=south east,
      fill=white,
      fill opacity=0.95,
      draw=gray!55,
      line width=0.4pt,
      text opacity=1,
      align=left,
      reverse legend,
    },
    scaled ticks=false,
    clip=false,
  },
  % New style that inherits from "nccl axis" but overrides x-axis and y-axis bounds
  nccl axis 16M/.style={
    nccl axis, % Inherits all properties defined above
    xmin=15000000, % Just below 16 MB (16,777,216) to ensure the first tick shows
    xtick={
      16777216, 67108864, 268435456, 1073741824, 4.294967296e9, 1.7179869184e10
    },
    xticklabels={
      16 MB, 64 MB, 256 MB, 1 GB, 4 GB, 16 GB
    },
    ymax=100, % Caps the Y-axis at 100
    ytick={0,25,50,75,100}, % Adjusts the Y-ticks to match the new max
  }
}

\definecolor{nvidia_green}{RGB}{118,185,0}
\definecolor{dark_green}{RGB}{60,120,0}
\definecolor{light_green}{RGB}{170,215,80}
\definecolor{dark_gray}{RGB}{94,94,94}
\definecolor{medium_gray}{RGB}{140,140,140}
\definecolor{light_gray}{RGB}{205,205,205}
\definecolor{dark_blue}{RGB}{0, 84, 159}
\definecolor{light_blue}{RGB}{100, 170, 225}
%% NVIDIA secondary palette
\definecolor{cpu_blue}{RGB}{0,113,197}
\definecolor{emerald}{RGB}{0,133,100}
\definecolor{amethyst}{RGB}{93,22,130}
\definecolor{fluorite}{RGB}{250,194,0}
\definecolor{garnet}{RGB}{137,12,88}

==> figures/source_based_routing_comparison/a2a_ew_sbr_spx_32N.tex <==
\begin{tikzpicture}
    \begin{axis}[nccl axis 16M, xmode=log, width=\linewidth,
        height=4.0cm,
        xticklabel style={rotate=40, anchor=east, font=\footnotesize},
        ylabel style={font=\footnotesize}]

    % dvora (out-of-place busbw from nvl_disabled_mask_dvora_results.log)
    \addplot[
      color=dark_gray,
      line width=1.75pt,
      mark=square*,
      mark size=1.5pt,
      mark options={solid, fill=white, draw=dark_gray, line width=1.2pt},
    ] coordinates {
      (16777216,22.38) (33554432,39.72) (67108864,60.41) (134217728,57.55)
      (268435456,55.27) (536870912,57.65) (1073741824,64.58) (2147483648,69.42)
      (4.294967296e9,65.93) (8.589934592e9,76.33) (1.7179869184e10,80.73)
    };
    \addlegendentry{ESR}

    % bdoris (out-of-place busbw from nvl_disabled_mask_bdoris_result.txt)
    \addplot[
      color=nvidia_green,
      line width=1.75pt,
      mark=*,
      mark size=1.5pt,
      mark options={solid, fill=nvidia_green},
    ] coordinates {
      (16777216,33.24) (33554432,48.45) (67108864,57.86) (134217728,66.71)
      (268435456,74.75) (536870912,83.24) (1073741824,88.78) (2147483648,90.77)
      (4.294967296e9,91.65) (8.589934592e9,92.04) (1.7179869184e10,92.56)
    };
    \addlegendentry{\projname}

    \end{axis}
\end{tikzpicture}


==> figures/source_based_routing_comparison/a2a_sbr_spx_28N_dvora.tex <==
\begin{tikzpicture}
\begin{axis}[nccl axis, xmode=log, width=0.4\textwidth,
    height=0.26\textwidth,]

% SBR
% Changed coordinates > 2.14 billion to scientific notation
\addplot[
  color=dark_gray,
  line width=1.75pt,
  mark=square*,
  mark size=1.5pt,
  mark options={solid, fill=white, draw=dark_gray, line width=1.2pt},
] coordinates {
  (130816,1.45) (261632,2.91) (523264,5.96) (1048320,11.27) (2096640,21.83)
  (4193280,39.23) (8388352,59.31) (16776704,76.16) (33553408,90.89) (67108608,83.41)
  (134217216,86.64) (268434432,68.97) (536870656,89.60) (1073741312,100.83)
  (2147482624,114.43) (4.29496704e9,126.78) (8.58993408e9,138.00) (1.717986816e10,143.04)
};
\addlegendentry{ESR}

% SP-X
% Changed coordinates > 2.14 billion to scientific notation
\addplot[
  color=nvidia_green,
  line width=1.75pt,
  mark=*,
  mark size=1.5pt,
  mark options={solid, fill=nvidia_green},
] coordinates {
  (130816,1.17) (261632,2.42) (523264,5.38) (1048320,10.12) (2096640,16.60)
  (4193280,34.48) (8388352,47.11) (16776704,68.08) (33553408,92.82) (67108608,95.33)
  (134217216,135.96) (268434432,160.41) (536870656,164.66) (1073741312,173.40)
  (2147482624,178.95) (4.29496704e9,181.57) (8.58993408e9,182.51) (1.717986816e10,182.40)
};
\addlegendentry{\projname}

\end{axis}
\end{tikzpicture}

==> figures/source_based_routing_comparison/a2a_sbr_spx_28N_ida.tex <==
\begin{tikzpicture}
    \begin{axis}[nccl axis, xmode=log, width=0.4\textwidth,
        height=0.26\textwidth,]

    % Cross-tier (no R), NCCL alltoall OOP bus bandwidth
    % Sizes ${>}2^{31}$ use scientific notation (same as a2a_sbr_spx_28N.tex)
    \addplot[
      color=dark_gray,
      line width=1.75pt,
      mark=square*,
      mark size=1.5pt,
      mark options={solid, fill=white, draw=dark_gray, line width=1.2pt},
    ] coordinates {
      (130816,1.38) (261632,2.85) (523264,5.75) (1048320,11.04) (2096640,21.10)
      (4193280,38.12) (8388352,57.96) (16776704,75.80) (33553408,96.84) (67108608,96.77)
      (134217216,142.34) (268434432,128.60) (536870656,150.85) (1073741312,155.79)
      (2147482624,113.35) (4.29496704e9,135.82) (8.58993408e9,151.30) (1.717986816e10,165.34)
    };
    \addlegendentry{ESR}

    % bdoris (SP-X / \projname), out-of-place bus bandwidth
    \addplot[
      color=nvidia_green,
      line width=1.75pt,
      mark=*,
      mark size=1.5pt,
      mark options={solid, fill=nvidia_green},
    ] coordinates {
      (130816,1.17) (261632,2.42) (523264,5.38) (1048320,10.12) (2096640,16.60)
      (4193280,34.48) (8388352,47.11) (16776704,68.08) (33553408,92.82) (67108608,95.33)
      (134217216,135.96) (268434432,160.41) (536870656,164.66) (1073741312,173.40)
      (2147482624,178.95) (4.29496704e9,181.57) (8.58993408e9,182.51) (1.717986816e10,182.40)
    };
    \addlegendentry{\projname}

    \end{axis}
\end{tikzpicture}

==> figures/time_to_ai/perf_under_failures.tex <==
\begin{tikzpicture}
  \begin{axis}[
    ybar,
    width=0.67\linewidth,
    height=3.7cm,
    bar width=10pt,
    ymin=0, ymax=105,
    ytick={0, 20, 40, 60, 80, 100},
    ylabel={All-to-All BW \\ (\% of line rate)},
    symbolic x coords={95pct, 80pct, 75pct},
    xtick={95pct, 80pct, 75pct},
    xticklabels={95\%, 80\%, 75\%},
    xlabel={Failed leaf available uplink capacity (\%)},
    title={\small\textbf{All-to-All Performance: One Leaf with Partial Uplink Failure}},
    axis x line*=bottom,
    axis y line*=left,
    ymajorgrids=true,
    grid style={dashed, gray!30},
    enlarge x limits=0.3,
    tick label style={font=\footnotesize},
    xlabel style={font=\small},
    ylabel style={font=\small, align=center},
    nodes near coords,
    every node near coord/.append style={font=\scriptsize, anchor=south},
    legend image code/.code={\fill[#1] (0,-0.07cm) rectangle (0.08cm,0.14cm);},
    legend columns=1,
    legend style={
      font=\scriptsize,
      at={(1.02,0.5)},
      anchor=west,
      xshift=0.5cm,
      fill=white,
      fill opacity=0.9,
      draw=gray!50,
      row sep=2pt,
    },
  ]

  % SOL (Black)
  \addplot[fill=black, draw=black] coordinates {
    (95pct,90) (80pct,82) (75pct,75)
  };
  \addlegendentry{Ideal}

  % SPX (Green)
  %\addplot[fill=nvidia_green, draw=nvidia_green] coordinates {
  %  (95pct,88) (80pct,78) (75pct,68)
  %};
  %\addlegendentry{\projname}

  % ETH (Gray)
  \addplot[fill=medium_gray, draw=medium_gray] coordinates {
    (95pct,70) (80pct,45) (75pct,25)
  };
  \addlegendentry{ETH}

  \end{axis}
\end{tikzpicture}


==> sections/design_principles_topology.tex <==
\subsection{Topology}
Modern AI clusters are scaling rapidly in both node count and per-node bandwidth,
which makes topology choice a first-order system decision rather than a
packaging detail\cite{meta_roce_lossless,microsoft_roce_lossless}. In this
section, we focus on the problem formulation and the key KPIs used to evaluate
topology options; concrete architectural choices are deferred to
Section~\ref{sec:design}. We use three explicit principles:
\begin{itemize}

    \item \textbf{Resiliency:} design the scale-out fabric so network failures
    have the minimal possible impact on running workloads.
    \item \textbf{Performance:} maintain high bisection bandwidth and low,
    predictable latency under bursty collective traffic.
    \item \textbf{Cost and power:} avoid unnecessary tiers, optics, and hops
    that inflate CapEx and energy per delivered bit.
    \item \textbf{Operational burden and readiness:} preserve a simple,
    repeatable operating model that remains robust as clusters scale to
    hyperscale deployment footprints.
\end{itemize}
This combination provides path diversity for failure resilience while keeping
the fabric practical to build and operate at giga-scale
\cite{meta_roce_lossless,microsoft_roce_lossless}.

==> sections/introduction.old.tex <==
\section{Introduction}


\ms{We would have liked to see a different structure: we discuss the problems:   
 (1) Unique workload requirements:  bursty fast collectives that requires fast convergence at sustained high network utilization. This is further challenging due to multi-job clusters, i.e., isolation is tough (2) Scaling cluster size and BW:  cant grow 3LFT due to added latency, challenges of a single port BW  (3) Building systems at large scale with low time-to-AI as an important requirement, as well as inevitability of failures at scale and the importance of seamless failover. (4) Operating large scale systems: the problem of performance/debugging large scale clusters  
All this should drive the reader to understand our main claims (1) HW-accelerated NW at switch and NIC - (1) SPCX -- HW per-packet load balancing, AR, CC separation (2)  Multiplane as a level on top -- HW NIC LB and the benefits of good LB in this scenario  (3)  perf debugging and real-world deployment experience.}

\subsection{Motivation: A Purpose-Built AI Fabric}
\ms{This motivation is a well known story. We are not in the first days of AI, so it feels redundant. Note that a lot of this has been published in the white paper two years ago, in very similar terms. So repeating this again will most likely piss off reviewers}



The rise of large-scale distributed AI has exposed a fundamental mismatch between the network infrastructure on which data centers were built and the communication patterns that AI workloads demand. Synchronous GPU collectives—all-reduce, reduce-scatter, all-gather, all-to-all—generate coordinated bursts of traffic that arrive simultaneously at switch ingress ports, saturate buffers instantaneously, and require every participating GPU to wait for the slowest transfer before computation can resume. In this regime, the performance of the entire cluster is determined not by mean network latency but by tail latency: the worst-case transfer time experienced by any single GPU in any single step.

Jitter -- variation in transfer completion time is therefore the defining enemy of AI networking performance. Jitter manifests in three forms that compound each other. Intra-job jitter arises when congestion within a single training job causes some GPUs to receive data later than others, stalling the collective. Inter-job jitter arises in multi-tenant deployments when congestion from a neighboring job backpressures into shared switch buffers, degrading throughput for jobs that played no part in generating the congestion. Latency jitter arises from variable queuing depth as the network alternates between underloaded and overloaded states. Eliminating all three forms of jitter—simultaneously, and without trading one for another—is the core mission of Spectrum-X Ethernet.
\ms{We do not have anything about jitter in the technical part of the paper. Here it sounds like a primary contribution, so we either add more focus on this in the experiments or tone it down}

Conventional off-the-shelf Ethernet cannot achieve this mission. Equal-Cost Multi-Path (ECMP) routing assigns entire flows to paths based on header hashes, leaving elephant flows—the dominant traffic type in AI workloads—unevenly distributed across the fabric. At scale, effective bandwidth utilization falls to 50–60\%. Priority Flow Control (PFC), the standard lossless mechanism, generates back-pressure that propagates hop by hop, causing head-of-line blocking that stalls unrelated flows. 

Neither mechanism can react to real-time congestion state at the microsecond timescales that collective synchronization demands.

\ms{this does not belong to the motivation. These are mechanisms in the design overview. And then once we say such things, we'll need to bring experimental evidence that these componets are those that work indeed. Also, we should be careful not to make it a marketing discussion with specific hardware makes}
Addressing these problems requires hardware acceleration at every layer of the network stack. Spectrum-X Ethernet achieves this through three co-designed hardware mechanisms:
\begin{itemize}
    \item Adaptive Routing (AR): per-packet path selection driven by real-time switch state, distributing individual packets across all available equal-cost paths to maximize utilization and eliminate hot spots.
    \item Congestion Control (CC): hardware telemetry from Spectrum-6 switches  \ms{will there be any discussion of what telemetry it is? Isn't it just ECN? It's been published in the white paper} is processed at line rate by the \ms{this is not for paper: ConnectX-9 Super}
    NIC, allowing the sender to reduce its rate before PFC thresholds are reached, suppressing pause propagation at the source.
    \item Packet-Level Balancing (PLB): hardware resequencing at the receiver restores in-order delivery after per-packet routing, making the load balancing mechanism fully transparent to RDMA semantics and collective communication libraries.
    \ms{Isn't PLB a multiplane tech for CC per plane and such?  }
\end{itemize}

Together, these mechanisms deliver a lossless fabric with deterministic, jitter-free performance—entirely in silicon, with no host device or CPU involvement in any performance-critical function.
\ms{NIC is a host device too. Isn't it involved?}


\subsection{What Is New: Giga-Scale Demands a New Topology Model}
Spectrum-X Ethernet was introduced at a time when large AI clusters comprised tens of thousands of GPUs. Two trends are rapidly changing the scale requirements that the network must meet.
First, cluster sizes are growing approximately $5\times$ per generation. The largest AI training jobs today operate on 100,000 GPUs or more, and the trajectory points toward 500,000 GPUs within a single coordinated fabric in the near term. Second, scale-out bandwidth per GPU is doubling annually as GPU compute throughput grows and models demand proportionally more inter-GPU communication. The NVIDIA Vera Rubin architecture provides 1.6 Tb/s of scale-out bandwidth per GPU, and successor platforms will demand more.

These two trends collide directly with the scaling limits of conventional multi-tier Clos topologies. Using state-of-the-art 102.4 Tbps switches, a two-tier fat-tree supports 2K GPUs; a three-tier topology reaches 64K GPUs. Reaching 128K GPUs at full bisection bandwidth requires a four-tier network. Each additional tier increases worst-case switch hop count, amplifying the tail latency that Spectrum-X Ethernet was built to eliminate. Deeper fabrics also multiply switch count, optical interconnect power, and operational complexity.
%—precisely when AI factories must maximize efficiency at every layer.

The answer is not to add more hierarchy. The answer is to add parallelism.
\ms{we are totally not the first to introduce multi-plane. We need to tone it down and add related work}

Multiplane topologies address this by decomposing each GPU’s NIC bandwidth into multiple lower-speed interfaces (e.g., 8$\times$200 Gb/s from a single 1.6 Tb/s ConnectX-9), each connecting into an independent network plane. Each plane is realized as a two-level fat tree. The full 128K GPU cluster is realized with only two switch tiers per plane; a 512K GPU factory using 8 planes and 4 rails requires only two tiers per plane. Maximum path length is capped at three switch hops regardless of cluster size, directly bounding tail latency.

Multiplane topology, however, introduces two distinct engineering challenges that must be solved together: how traffic is distributed across planes, and how the topology handles failures.

For traffic distribution, a naive approach is to partition collective operations across planes at the host or software level, assigning different message transfers to different planes through explicit scheduling in the collective library or transport stack. Such host-based approaches distribute load at message or connection granularity and make scheduling decisions before packets enter the fabric -- without visibility into real-time switch congestion state. More critically, host-based approaches reintroduce the jitter that Spectrum-X Ethernet was designed to eliminate: any time a load-balancing or failure-recovery decision is made in the host, it operates on host device or host CPU timescales (microseconds to milliseconds) rather than hardware timescales (sub-microsecond) \ms{we don't have any backing for that. We are submilliseconds, but definitely not submicro}. 
%The result is performance variability at exactly the synchronization points where GPUs wait for each other. 

Spectrum-X Ethernet solves the load balancing challenge entirely in hardware. The \ms{drop:ConnectX-9 Super}
NIC distributes each GPU’s traffic across all active planes in real time, per packet, informed by continuous telemetry from Spectrum-6 switches \ms{can we say what this telemetry does?}. Packet resequencing at the receiver is performed in the NIC ASIC before any data reaches the RDMA layer, making multiplane distribution transparent to applications and collective libraries. Congestion within a plane is detected and addressed in hardware before it can generate backpressure, and traffic is redistributed across planes preemptively. No protocol modifications are required; full RDMA semantics are preserved. 

==> sections/lessons-learned-backup-2026-04-13.tex <==
\section{Lessons Learned}


Operating Spectrum-X Ethernet at scale across large AI factories has produced a concrete set of design conclusions. These lessons informed the multiplane architecture and reinforce why hardware acceleration is the only viable path to jitter-free AI networking.

\ms{For every case we need to have a concrete example which shows how this lesson comes into play in a real deployment}

\ms{can we talk why some design decisions were very important? }

\subsection{Lossless Fabric Is Essential}
Packet loss is not a latency tax—it is a synchronization barrier. At scale, a single dropped packet forces retransmission that stalls the receiving GPU. Through collective synchronization, every other GPU in the job waits. The cost of one lost packet is not one retransmission delay; it is that delay multiplied by the collective size. Any architecture that accepts packet loss as a steady-state operating point—trading congestion avoidance for simpler load balancing—does not eliminate jitter: it substitutes one source of tail latency for another. Lossless operation through hardware-controlled ECN and PFC is a foundational requirement, not a feature.

\subsection{Multiplane }





\subsection{Debugging and  }


These lessons come from operating and tuning large-scale AI Ethernet fabrics in
production. The common theme is operational predictability: when behavior is
deterministic, bottlenecks are easier to isolate, performance is easier to
improve, and reliability is easier to maintain at scale.


\subsection{AR Symmetry Enables Anomaly Detection and Debugging at Scale}
Hardware adaptive routing produces a structurally symmetric traffic pattern across the fabric. AR traffic is evenly distributed across equivalent links, even at short time scales. This creates a clear baseline for operations: abnormal behavior
appears immediately as a visible asymmetry in counters such as bandwidth, buffers, or PFC. This behavior facilitates identifying anomalous patterns, and teams
can localize misconfigurations or failing elements quickly.

Anomalies such as a blocked link, a misconfigured switch, or a failing component manifest as measurable asymmetries in switch-level counters and bandwidth histograms, making them detectable without application-level instrumentation. 

Real deployments at scale have demonstrated that symmetry-based anomaly detection can localize hardware failures and congestion events to the specific fabric element responsible—a diagnostic capability that depends entirely on the uniform distribution property that hardware AR provides. Host-driven forwarding breaks this symmetry, obscuring the fabric’s state and complicating root-cause analysis.

\ms{we need a concrete graphic example when asymetry is apparent and how it is expressed }


\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{figures/traffic_balance_ar.png}
    \caption{Mean BW over a 5 minute window in hash-based routing (left) and adaptive-routing (right) \ms{nice picture but what does it have to do with the lessons?}}
    \label{fig:ar_vs_non_ar_load_balance}
\end{figure}


\subsection{Straggler detection is key and network telemetry is a powerful asset}
At large scale, end-to-end job performance is often dictated by a small number
of stragglers rather than by average behavior. Detecting these stragglers is in non-trivial in the general case, and network telemetry can be used to detect even non-network-related issues.

Basic manual techniques includes:

\ms{The fact the telemetry is helpful is a "known truth". What's surprising? What does facilitate straggeler detection in SPCX specifically? Is there anything that makes it architecturally simpler, like symmetries?}
\begin{itemize}
  \item NICs sending PFCs
  \item Non-bimodal bandwidth histograms, with significant sub-line-rate periods.
  \item Anomalous leaf downlinks buffer histograms
\end{itemize}

\ms{what about gray failures?}

\subsection{HFT is crucial for profiling and perf tuning}
\ms{1. need example, 2. HFT needs to be explained better. 3. the mechanism itself and what it can help with. How is this lesson learned? }
High-frequency telemetry (HFT) exposes network dynamics at the timescale where
performance problems actually occur. Sub-millisecond visibility into queueing dynamics, pause behavior, and path utilization enables precise profiling and
targeted tuning of congestion-control and adaptive-routing parameters, under ever-evolving workload demands.

Additionally, HFT is used for measuring convergence times in dynamic failure scenarios, and identifying BW jitter or sub-line-rate plateaus.

\subsection{High-Frequency Telemetry Is Required for Job Performance Visibility}
Step-time degradation in large training jobs correlates directly and causally with congestion events in the fabric. Detecting this correlation—and acting on it before it compounds across multiple training steps—requires telemetry at the frequency of the network events themselves, not at the polling intervals of management software. Spectrum-X Ethernet’s high-frequency telemetry (HFT) captures per-switch congestion signals, NIC pause events, and bandwidth utilization at sub-millisecond granularity, enabling correlation between step-time anomalies and their network-level root cause in real time. This has proven essential for diagnosing and tuning congestion control parameters in production deployments, and for distinguishing between application-layer effects (collective library behavior, garbage collection pauses) and network-layer effects (congestion, retransmissions, PFC pause propagation).





\subsection{No congestion spreading? }
\ms{can we say something like we experienced no such things, it's not a problem? }

\subsection{Job allocation agnostic}
\ms{what is the lesson? That this was very importnat design decision?}
A robust fabric should deliver predictable behavior regardless of where a job is
placed. Production experience shows this promise is fulfilled by SpectrumX in practice. This
allocation-agnostic behavior reduces scheduling constraints, improves cluster
utilization, and increases predictability.

\subsection{Importance of telemetry consolidating across NIC, switch, scheduler, and application}
No single telemetry stream is sufficient for root-cause analysis. Accurate
diagnosis requires a unified, time-aligned view across NIC signals, scheduler
context, switch fabric counters, and application performance measurements.
As an example let us consider a bad link that sees symbol errors. The NIC will show retransmissions, the switch will show where the packets were dropped, and the scheduler will identify the affected tenant and job. The application metric, such as training step time, will allow us to assess the practical impact and prioritize mitigation accordingly.

For example, workload analysis of modern inference workloads has shown that different communication kernels—scheduled collective operations versus asynchronous one-sided puts—produce fundamentally different traffic patterns, bandwidth utilization levels, and NIC pause rates, even when running the same model on the same hardware. An end-to-end telemetry platform that exposes all layers together is not a debugging convenience; it is a prerequisite for understanding and optimizing AI fabric performance.

\ms{example???}



\subsection{Hardware Adaptive Routing Delivers Uniform Bandwidth Distribution}
A key insight from production deployments is that the uniformity of bandwidth distribution across the fabric is as important as the total available bandwidth. Hardware-based adaptive routing (AR), operating per-packet with real-time visibility into switch queue state, produces consistent, balanced utilization across all fabric levels—leaf uplinks, spine downlinks, and inter-tier links—even under the synchronized burst patterns of large GPU collectives. Approaches that perform path selection on the host, without live telemetry from the switch fabric, cannot achieve this uniformity: decisions made at connection setup or message granularity do not reflect actual congestion state at the time packets traverse the network, resulting in skewed utilization, hot spots, and performance variability that is difficult to predict or bound.



Taken together, these lessons point to a single architectural conclusion: jitter-free AI networking at giga-scale requires hardware acceleration at every layer—adaptive routing, congestion control, telemetry collection, and multiplane load balancing—all operating at the timescales of the network itself. The remainder of this paper describes the Spectrum-X Ethernet multiplane architecture that realizes these principles and presents measured results from production deployments.



==> sections/lessons-learned.tex <==
\section{Lessons Learned - Gilad}

Summarize practical lessons, pitfalls, and insights from building and
using the system.






